You Are What You Say: Exploiting Linguistic Content for VoicePrivacy Attacks

Speaker anonymization systems hide the identity of speakers while preserving other information such as linguistic content and emotions. To evaluate their privacy benefits, attacks in the form of automatic speaker verification (ASV) systems are employed. In this study, we assess the impact of intra-speaker linguistic content similarity in the attacker training and evaluation datasets, by adapting BERT, a language model, as an ASV system. On the VoicePrivacy Attacker Challenge datasets, our method achieves a mean equal error rate (EER) of 35%, with certain speakers attaining EERs as low as 2%, based solely on the textual content of their utterances. Our explainability study reveals that the system decisions are linked to semantically similar keywords within utterances, stemming from how LibriSpeech is curated. Our study suggests reworking the VoicePrivacy datasets to ensure a fair and unbiased evaluation and challenge the reliance on global EER for privacy evaluations.

==> Figures/text_based_attack.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw[shift={(128, 764)}, xscale=0.1875, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \draw[shift={(108, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center]
     at (100, 736) {Input text};
  \node[ipe node, rotate=90, anchor=center]
     at (140, 736) {Tokenizer};
  \begin{scope}[shift={(24, -13.5155)}]
    \node[ipe node, anchor=center]
       at (184, 692) {Encoding};
    \node[ipe node, anchor=center]
       at (184, 704) {Positional};
  \end{scope}
  \begin{scope}[shift={(-100.8792, -216.3119)}, xscale=1.2361, yscale=1.309]
    \draw
      (224, 700) circle[radius=8.9443];
    \begin{scope}[shift={(2, 0)}]
      \draw
        (216, 700)
         arc[start angle=180, end angle=360, x radius=3, y radius=-4];
      \draw
        (222, 700)
         arc[start angle=180, end angle=360, x radius=3, y radius=4];
    \end{scope}
  \end{scope}
  \node[ipe node, anchor=center, font=\large]
     at (176, 736) {$\oplus$};
  \draw[shift={(152, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[->]
    (176, 712)
     -- (176, 732);
  \draw[shift={(260, 700)}, rotate=90, xscale=0.5625, yscale=0.4375]
    (0, 0) rectangle (128, -64);
  \draw[shift={(180, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(308, 716)}, rotate=90, xscale=0.3125, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (320, 736) {Pooler};
  \draw[shift={(288, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (301.955, 762.531) {$(\text{B}, \text{L}, 768)$};
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (345.955, 762.531) {$(\text{B}, 1, 768)$};
  \draw[shift={(332, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(352, 708)}, rotate=90, xscale=0.4375, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (364, 736) {Classifier};
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (389.955, 762.531) {$(\text{B}, 1, 921)$};
  \draw[shift={(376, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center]
     at (445.925, 736) {Speaker Logits};
  \draw[shift={(200, 764)}, xscale=0.1563, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (210, 736) {LayerNorm};
  \draw[shift={(220, 764)}, xscale=0.1563, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (230, 736) {Dropout};
  \draw[shift={(240, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center, font=\small]
     at (268.304, 736) {(12 x)};
  \node[ipe node, rotate=90, anchor=center]
     at (280.304, 736) {BERT Layer};
  \draw[shift={(396, 700)}, rotate=90, xscale=0.5625, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (408, 736) {AAM-Softmax};
  \draw[shift={(420, 736)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
\end{tikzpicture}


==> Figures/text_based_attack_enroll.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw[shift={(136, 776)}, xscale=0.1875, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \draw[shift={(116, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center]
     at (100, 748) {Enrolment utt.};
  \node[ipe node, rotate=90, anchor=center]
     at (148, 748) {Tokenizer};
  \begin{scope}[shift={(32, -1.5155)}]
    \node[ipe node, anchor=center]
       at (184, 692) {Encoding};
    \node[ipe node, anchor=center]
       at (184, 704) {Positional};
  \end{scope}
  \begin{scope}[shift={(-92.879, -204.312)}, xscale=1.2361, yscale=1.309]
    \draw
      (224, 700) circle[radius=8.9443];
    \begin{scope}[shift={(2, 0)}]
      \draw
        (216, 700)
         arc[start angle=180, end angle=360, x radius=3, y radius=-4];
      \draw
        (222, 700)
         arc[start angle=180, end angle=360, x radius=3, y radius=4];
    \end{scope}
  \end{scope}
  \node[ipe node, anchor=center, font=\large]
     at (184, 748) {$\oplus$};
  \draw[shift={(160, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[->]
    (184, 724)
     -- (184, 744);
  \draw[shift={(268, 712)}, rotate=90, xscale=0.5625, yscale=0.4375]
    (0, 0) rectangle (128, -64);
  \draw[shift={(188, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(316, 728)}, rotate=90, xscale=0.3125, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (328, 748) {Pooler};
  \draw[shift={(296, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (309.96, 782.531) {$(\text{N}_{enroll}, \text{L}, 768)$};
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (353.96, 782.531) {$(\text{N}_{enroll}, 1, 768)$};
  \draw[shift={(340, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(360, 720)}, rotate=90, xscale=0.4375, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (372, 748) {Classifier};
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (397.96, 782.531) {$(\text{N}_{enroll}, 1, 921)$};
  \draw[shift={(384, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(208, 776)}, xscale=0.1563, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (218, 748) {LayerNorm};
  \draw[shift={(228, 776)}, xscale=0.1563, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (238, 748) {Dropout};
  \draw[shift={(248, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center, font=\small]
     at (276.3, 748) {(12 x)};
  \node[ipe node, rotate=90, anchor=center]
     at (288.3, 748) {BERT Layer};
  \node[ipe node, rotate=90, anchor=center]
     at (112, 748) {Input text};
  \node[ipe node]
     at (96, 800) {(for each enrollment speaker)};
  \draw[shift={(404, 720)}, rotate=90, xscale=0.4375, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (416, 748) {Average};
  \draw[shift={(428, 748)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (441.96, 774.531) {$(1, 1, 921)$};
  \node[ipe node, rotate=90, anchor=center]
     at (460, 748) {enrolment embedding};
\end{tikzpicture}


==> Figures/text_based_attack_trial.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw[shift={(144, 768)}, xscale=0.1875, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \draw[shift={(124, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center]
     at (108, 740) {Trial utt.};
  \node[ipe node, rotate=90, anchor=center]
     at (156, 740) {Tokenizer};
  \begin{scope}[shift={(40, -9.5155)}]
    \node[ipe node, anchor=center]
       at (184, 692) {Encoding};
    \node[ipe node, anchor=center]
       at (184, 704) {Positional};
  \end{scope}
  \begin{scope}[shift={(-84.879, -212.312)}, xscale=1.2361, yscale=1.309]
    \draw
      (224, 700) circle[radius=8.9443];
    \begin{scope}[shift={(2, 0)}]
      \draw
        (216, 700)
         arc[start angle=180, end angle=360, x radius=3, y radius=-4];
      \draw
        (222, 700)
         arc[start angle=180, end angle=360, x radius=3, y radius=4];
    \end{scope}
  \end{scope}
  \node[ipe node, anchor=center, font=\large]
     at (192, 740) {$\oplus$};
  \draw[shift={(168, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[->]
    (192, 716)
     -- (192, 736);
  \draw[shift={(276, 704)}, rotate=90, xscale=0.5625, yscale=0.4375]
    (0, 0) rectangle (128, -64);
  \draw[shift={(196, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(324, 720)}, rotate=90, xscale=0.3125, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (336, 740) {Pooler};
  \draw[shift={(304, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (317.96, 766.531) {$(1, \text{L}, 768)$};
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (361.96, 766.531) {$(1, 1, 768)$};
  \draw[shift={(348, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(368, 712)}, rotate=90, xscale=0.4375, yscale=0.375]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (380, 740) {Classifier};
  \node[ipe node, rotate=90, anchor=base, font=\small]
     at (405.96, 766.531) {$(1, 1, 921)$};
  \draw[shift={(392, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \draw[shift={(216, 768)}, xscale=0.1563, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (226, 740) {LayerNorm};
  \draw[shift={(236, 768)}, xscale=0.1563, yscale=0.875]
    (0, 0) rectangle (128, -64);
  \node[ipe node, rotate=90, anchor=center]
     at (246, 740) {Dropout};
  \draw[shift={(256, 740)}, xscale=0.625, ->]
    (0, 0)
     -- (32, 0);
  \node[ipe node, rotate=90, anchor=center, font=\small]
     at (284.3, 740) {(12 x)};
  \node[ipe node, rotate=90, anchor=center]
     at (296.3, 740) {BERT Layer};
  \node[ipe node, rotate=90, anchor=center]
     at (120, 740) {Input text};
  \node[ipe node]
     at (104, 792) {(for each trial utterance)};
  \node[ipe node, anchor=base, font=\small]
     at (383.717, 692.288) {$(\text{N}_\text{enroll\_spk}, 1, 921)$};
  \draw[->]
    (384, 700)
     -- (384, 704)
     -- (400, 704)
     -- (400, 724)
     -- (412, 724);
  \begin{scope}[shift={(-4, 0)}]
    \draw
      (416, 748) rectangle (472, 716);
    \node[ipe node, anchor=center]
       at (444, 738) {Cosine};
    \node[ipe node, anchor=center]
       at (444, 726) {Distance};
  \end{scope}
  \node[ipe node, anchor=base]
     at (384, 676) {Enrollment Embeddings};
\end{tikzpicture}

